Representation as a Service

Consider a Machine Learning Service Provider (MLSP) designed to rapidly create highly accurate learners for a never-ending stream of new tasks. The challenge is to produce task-specific learners that can be trained from few labeled samples, even if tasks are not uniquely identified, and the number of tasks and input dimensionality are large. In this paper, we argue that the MLSP should exploit knowledge from previous tasks to build a good representation of the environment it is in, and more precisely, that useful representations for such a service are ones that minimize generalization error for a new hypothesis trained on a new task. We formalize this intuition with a novel method that minimizes an empirical proxy of the intra-task small-sample generalization error. We present several empirical results showing state-of-the art performance on single-task transfer, multitask learning, and the full lifelong learning problem.

==> chapters/discussion.tex <==
%!TEX root = ../ldr.tex

In this paper, we introduced a meta-algorithm that addresses the problem of learning in online environments with streaming tasks and high dimensional inputs. Our meta-algorithm relies on altering a feature representation to make its output useful as a preprocessor for data on a new task. The flexibility of our algorithm is in its modularity, as the function approximator can be a regressor, a classifier or a ranker. The representation can also be changed to suit different domains. Simple representations like boosted stumps, or even complex ones like convolutional networks are trainable with our method. We tested our algorithm in three relevant contexts: Representation learning, multitask learning and lifelong learning. In the representation learning case, we show how our model can be used to train complex representations like convolutional nets and significantly outperform similar nets trained by backprop. In the multitask learning case, we show that our framework, despite not retaining information specific to any task it has seen before, performs comparably to state-of-the-art multitask learning algorithms. Finally, in the lifelong learning scenario, we show how our algorithm outperforms ELLA in environments of streaming tasks with relatively low dimensionality and how it provides large gains in high dimensional regimes compared to single task learners.

==> chapters/evaluation.tex <==
%!TEX root = ../ldr.tex
We evaluate our method in three different contexts, selected to reflect a range of transfer settings. 

 Third we tackle the full lifelong learning problem, where we show how LeaDR compares to state-of-the-art methods in situations where the number of training tasks is large and testing is done on different problems than training, as in the MLSP problem.

\subsection{Representation Learning for Single Task Transfer}
First we consider the single task transfer case, with the goal of showing that LeaDR provides a robust solution for supervised transfer to new tasks. This experiment targets the NIPS 2011 transfer learning challenge \cite{nips_challenge_2011}. 
Data is available as follows: a first dataset of 50,000 $32 \times 32 \times 3$ images labelled into 100 classes is given (namely, the CIFAR-100 dataset \cite{krizhevsky2009learning}), along with a second dataset of 100,000 unlabelled $32 \times 32 \times 3$ images. The target domain is a 10-way classification problem, for which only 120 labelled training examples are given; each of the classes in this target domain is distinct from those seen in the two larger datasets. The goal is to create a method that performs as well as possible on the target domain's test set, which contains another 2542 samples. The best previously published result for this challenge was Spike and Slab Sparse Coding (S3C) \cite{goodfellow2012large} which ignores the labels on CIFAR-100 and uses it just as unlabelled data. After training, the representation learned by S3C is used to extract features, on which a linear classifier is trained on the 120 samples.

To instantiate the LeaDR framework, we used a convolutional neural network for the representation stage and logistic regression (trained by gradient descent) for the supervised task-specific learner.  A stream of training tasks was simulated by sampling $K=30$ different  20-way classification problems from the CIFAR-100 dataset.  The final training task presented is the target task (120 or fewer examples); we used the supervised learner from this task to predict labels for the target test set (2542 examples).   We compare this to a standard convolutional network trained by backpropagation with the full labelled CIFAR-100 dataset and the few examples from the target task. Note that for vision tasks, these convolutional architectures present a remarkably strong baseline as pointed out by \cite{razavian2014cnn}. For both of these methods, we ignore the unlabelled data. More implementation details are in the supplementary material.

\begin{wrapfigure}{r}{0.6\textwidth}
  \includegraphics[scale=0.8]{materials/challenge_lr.pdf}
  \caption{NIPS 2011 transfer learning challenge}
\end{wrapfigure}

Figure 2 depicts how our algorithm performs against backpropagation as the number of samples per class increases. Our algorithm depicts considerable improvement when training on upto 30 samples. Specifically, on the important ``one shot'' case, our algorithm presents a gain of about 8\% compared to backprop. Note that with 5 samples per class, supervised representations outperform unsupervised ones. Surprisingly, for the net trained with standard backprop, the performance worsens slightly as we train on the whole 120 samples. We believe this is due to the uneven distribution of 120 samples among the 10 classes on the test problem. The gains our algorithm has in small sample cases showcase the advantage of minimizing empirical generalization as opposed to standard loss.

\subsection{Representation Learning for Multitask Transfer}
Second we focus on the standard multitask learning case, where the training tasks are fixed and testing tasks are constrained to be from the same set of tasks (though LeaDR cannot exploit this information).   We empirically show that even though our model was not made for multitask learning and does not assume task correspondence, it compares favorably to state-of-the-art multitask learners.

We consider two problems that are standard in the multitask learning literature:  the Landmine \cite{xue2007multi} and London schools \cite{kumar2012learning} datasets, both taken from \cite{ruvolo2013ella}\footnote{A third dataset used in that paper was not available, despite our efforts to have access to it.}. The Landmine dataset is a multitask classification problem and the London schools is a multitask regression problem. Both datasets are fairly low dimensional.   We compare our method to two algorithms specifically designed for multitask learning: GOMTL \cite{kumar2012learning}, and OMTL \cite{saha2011online}, as well as the lifelong learning algorithm ELLA \cite{ruvolo2013ella}. We also include comparison to standard single task learning (STL) as a baseline: logistic regression for the Landmine (classification) problem and random forests for the London schools (regression) problem. We apply the experimental methodology used in~\cite{ruvolo2013ella}, where data for each task (within a domain) is split 50/50 between training/testing sets.  We measure error on Landmine (classification) in terms of Area Under the Curve (AUC)\footnote{The choice of AUC as opposed to standard misclassification error is to conform with \cite{ruvolo2013ella}. In our experiments, misclassification error was about the same for all the methods, including STL. In our opinion, this suggests the Landmine dataset may not be a great domain for multitask learning.}. For the London schools (regression), we measure error in RMSE.   More details on the datasets, training process and experimental setup are in the supplemental material.

\begin{table}[!htp]
\caption{Performance of LeaDR (our method) against standard multitask transfer learning datasets. }
\vspace{2mm}
\centering
    \begin{tabular}{l|c|c|c|c|c|c|c}	
    \textbf{Dataset}        & \textbf{Error Type} & \textbf{OMTL} & \textbf{GOMTL} & \centering \textbf{ELLA}  & \textbf{LeaDR} & \textbf{Baxter} & \textbf{STL} \\ \hline
     Landmine      & AUC & 0.63   & 0.78 & 0.776 &  0.78 & 0.74 & 0.76           \\
     London Schools & RMSE & N/A  & 10.10 & 10.20 & 10.08 & 0000 & 11.06       \\
    \end{tabular}
\end{table}

Table 1 summarizes the results, showing that LeaDR compares favourably to other state-of-the-art algorithms on these multitask learning datasets. We note that, due to the simplicity of these datasets in terms of task specification and observation dimensionality, most reasonable methods perform rather similarly, as there is little room to gain relative to basic single task learning. Our final experimental setting is intended to move past some of these limitations, to examine performance in a setting that more closely approaches the intent of online transfer learning with streaming tasks and high dimensional problems.

\subsection{Lifelong Learning Experiments}

%\begin{wrapfigure}{r}{0.6\textwidth}
%  \includegraphics[scale=0.8]{materials/challenge_lr.pdf}
%  \caption{NIPS 2011 transfer learning challenge}
%\end{wrapfigure}


We now examine how our algorithm performs in the context of lifelong learning where tasks stream in an online manner. In this scenario, algorithms are trained on a long sequence of tasks, where each task is presented only once. After training, error is measured on a set of new tasks not seen during training.

We simulate the online streaming of tasks by sampling 1000 random 5-way classification problems from the set of 20 classes of the newsgroups dataset \cite{20_newsgroups}. After training, we present 100 5-way classification problems to each algorithm, each problem represented by a small set of labelled samples. Each algorithm creates a hypothesis for each testing problem, the accuracy of each hypothesis is measured on a test set for that particular problem. Samples used for training the algorithms, for representing the test problems and for measuring the accuracy of each hypothesis come from three disjoint sets.

We instantiate our method with two layer neural net for the representation and a logistic regression for the function approximator. We compare our method to ELLA \cite{ruvolo2013ella} and single-task multinomial logistic regression. The restriction of our comparison to ELLA is mainly because algorithms like \cite{saha2011online,kumar2012learning} can't operate efficiently when the number of tasks is as high.

%\begin{figure}[htp]
% \subfigure[$d=10$]{\includegraphics[width=4.5cm]{materials/newsgroups_ll_10.pdf}}
%  \subfigure[$d=100$]{\includegraphics[width=4.5cm]{materials/newsgroups_ll_100.pdf}}\hspace{-.4em}
%  \subfigure[$d=2000$]{\includegraphics[width=4.5cm]{materials/newsgroups_ll_2000.pdf}}\hspace{-.4em}
% 
%  \caption{Results for the lifelong learning experiments on the 20-newsgroups dataset. $d$ is the number of dimensions for each document.}
%\end{figure}


\begin{figure}[hctp]
\hspace*{-.3in}
 \subfigure[c][Results on CIFAR-100 ]
 {\includegraphics[width=15cm]{materials/cifar_ll_all.pdf}}

 \subfigure[c][Results on 20-newsgroups]{\includegraphics[width=14cm]{materials/newsgroups_ll_all.pdf}}
 \caption{Results for the lifelong learning experiments. $d$ is the number of dimensions in the input.}
\end{figure}

%\begin{figure}
%\hspace*{-.2in}
%\includegraphics[width=15cm]{materials/cifar_ll_all.pdf}
%\end{figure}
%%


Since ELLA is not efficient for problems with high input dimensions, we are restricted to low and medium dimensional problems when comparing to it. In high dimensional settings, we compare our algorithm to logistic regression since we are not aware of any algorithms that operate in this setting. To construct the low and medium dimensional settings, we project documents in the 20 newsgroups dataset onto 10 and 100 dimensions respectively by using LDA \cite{blei2003latent}. To construct the higher dimensional problem, we represent each document by a vector of counts for the 2000 most-common non-stop words. Figure 3 presents the accuracy of each method as the number of samples for testing tasks increases. Each point in figure 3 was averaged over the 100 different problems and over 10 different sample sets for each test task. We also run the same experiment on a stream created from CIFAR 100. In this case, we project down using PCA to create lower dimensional problems.

As depicted in Figure 3, our method outperforms ELLA significantly on every sample size, particularly in regions where the new task is represented with a small number of samples. Surprisingly, single-task logistic regression sometimes outperforms ELLA in this setting. Note that our algorithm's performance on different problems was consistent, whereas ELLA had a much higher variance. Moreover, on the 20 newsgroups, all algorithms gain little by moving from 10 to 100 dimensions, but when moving from 100 to 2000 dimensions, our algorithm depicts significant gains. In the case for CIFAR 100, similar behaviour is depicted. Note that since our algorithm can leverage complex representations like convolutional nets, for high dimensional tasks like CIFAR 100, this proves quite useful. To the best of our knowledge, this paper is the first to test in this particular setting.

==> chapters/introduction.tex <==
%!TEX root = ../ldr.tex

Machine learning practitioners are often challenged with tasks for which few labeled samples exist. These include tasks for which data is expensive to label (e.g., medical images) and tasks where it is physically impractical to obtain large amounts of labeled data (e.g., human computer interaction). When facing such tasks, there are generally three paths towards acceptable performance: 
\begin{enumerate}
\item Using domain knowledge.
\item Using unlabeled samples.
\item Using labeled samples from a different, but related task.
\end{enumerate}

Bayesian methods \cite{fei2007learning} have typically focused on the first option, by using knowledge of structure in the target task to bias search towards better hypotheses. Other methods, like manifold regularization \cite{belkin2006manifold}, blend the first and second options by combining domain knowledge, like an engineered distance metric/kernel, and unlabeled samples. Meanwhile, the representation learning community has emphasized learning from unlabeled data with as little domain knowledge as possible. A number of methods like Deep Boltzmann Machines \cite{salakhutdinov2009deep}, Stacked Denoising Autoencoders \cite{vincent2010stacked}, and Sparse Coding \cite{raina2007self} have proven effective for transfer from unlabeled data to tasks with few labeled samples. Representations learned by such methods can either be used directly on new tasks or fine-tuned on new tasks using their labeled training data.

While methods based on options (1) and (2) work relatively well for a variety of tasks, they typically ignore the existence of large amounts of labeled data from different, but possibly related tasks that may provide significant information about the task-of-interest. The transfer learning community has sought to leverage this idea through a variety of methods generally categorized as ``supervised transfer'' methods. The most common tools for supervised transfer come from multitask learning \cite{caruana1997multitask}, in which a fixed set of tasks is given a priori and the learner seeks a model that can \textit{generalize well to new samples} from the given tasks. While multitask learning has been effective in many situations, it falls short in environments where new tasks are constantly arriving and one seeks to \emph{generalize well to new tasks} as they arrive. This more challenging type of transfer is generally referred to as inductive bias learning \cite{baxter2000model}, lifelong learning \cite{thrun1995lifelong}, learning to learn \cite{thrun1996learning}, or never ending learning \cite{carlson2010toward}, among other names. Our work focuses on this last setting.

%Most transfer learning methods concern themselves with situations when data on the target domain is scarce. This is because the gain from transfer diminishes as more data is available in the target domain. Interest in such data scarce regimes is well justified from a practical point of view, as in many situations we are restricted to small amounts of data. Examples of such situations include those in which data is expensive to label (e.g, medical images) to those where it is practically infeasible to obtain large amounts (e.g, human computer interaction).

%To illustrate the setting we are interested in, imagine a Machine Learning Service Provider (MLSP) facing a continuous stream of tasks with the same input domain, but with output domains that may differ. Each new task is presented to the MLSP implicitly through a small batch of labeled examples. For each presented task the MLSP seeks to learn a new function approximator that generalizes well, i.e.~minimizes test error, on the task. To succeed, the MLSP needs a representation of its input domain that permits effective learning from only a few samples. 

%The setting we consider in this paper, is that of a Machine Learning Service Provider (MLSP) whose service is customized face recognition. Users present the MLSP with small sets of faces labeled as ``friend'' or ``foe'', and the MLSP tries to provide each user with a classifier that can be used to distinguish friend from foe. If the MLSP has a good representation of face-space, it should be able to produce effective classifiers even though: each user may only present a small amount of labeled data, new users will constantly be joining the service, existing users may reconsider their allegiances, and friend/foe labels will certainly be inconsistent across users. This final point is particularly troublesome as it precludes direct transfer of friend/foe labels between users. That is, the labels provided by each user are not in correspondence (i.e.~my friend $\neq$ your friend and my foe $\neq$ your foe). We will refer to this particular problem as ``task correspondence''.

The setting we consider in this paper is that of a Machine Learning Service Provider (MLSP), whose service is creating highly accurate, customized face recognizers. A client, for instance a video surveillance company, would present our MLSP with a small set of labelled faces, requesting our MLSP to create an accurate classifier for that particular problem. This set could be a simple problem (e.g., employee vs. not employee), or a complex one (e.g., recognize all employees). If the MLSP has a good representation of face-space, it should be able to produce effective classifiers even though: each client may only present a small amount of labeled data, new clients will constantly be joining the service, and labels will be inconsistent across clients (i.e., one company's person of interest is not another's). This final point is particularly troublesome as it precludes direct transfer of label information between clients. That is, the labels provided by each client are not in correspondence. We will refer to this particular problem as ``task correspondence''.


Scaling will also be an issue for our MLSP, as the number of presented tasks could be large enough that the memory and computational requirements of a practical algorithm, when dealing with a constant stream of tasks, would need to be sublinear in the number of previously-presented tasks. While some work has sought to address problems similar to our proposed MLSP (e.g., \cite{saha2011online, ruvolo2013ella}), the resulting algorithms have suffered from poor scaling with respect to the number of tasks and/or the input dimensionality. Thus, experimental results for these algorithms has focused on relatively simple multitask learning problems. Note that multitask learning does not face the ``task correspondence'' problem, as multitask learning usually assumes that labels provided with the training samples correspond directly to the labels to be predicted for unseen samples.

%On example of such MLSP is a website which directs users to available information (e.g.~blog posts, news articles, etc.) based on their observed history of likes/dislikes for information they have already seen. In this case, new users may continually join the site with only a minimal amount of like/dislike information made available a priori, and new information may continually become available. Intuitively, one might assume that there exists some ``coarsest-common-partition (CCP)'' of the set of available information sources such that the users' binary partitions of information space into things they like or dislike can be approximated by binary partitions that do not further divide any elements of the CCP. If our MLSP could learn about the structure of the CCP from the likes and dislikes of its users, its performance could improve dramatically. This performance would be depicted by providing better recommendations to existing users and by more rapidly accommodating new users and new information sources.

In this paper, we present an approach to lifelong learning problems like that faced by our MLSP. Our method is efficient in both the input dimension and the number of presented tasks. We build on the intuition that good representations should enable strong generalization on new tasks from only a small number of labeled samples. Our method operates on a given parametric feature extractor and a given function approximator training algorithm by manipulating the feature extractor, through its parameters, to minimize an empirical proxy for the generalization error of function approximators trained on the features it extracts.

While initially motivated by learning representations for inter-task transfer from a large stream of tasks, the algorithm we propose can also improve transfer to new tasks when learning from just a single encountered task. Thus, our work is connected to a recent phenomenon in the computer vision community wherein deep neural networks are trained on a single highly multiclass task with large amounts of labeled data, after which the features learned by the networks are applied to tasks other than the training task, for which few labeled samples are available \cite{razavian2014cnn, Jia13caffe, donahue2013decaf}. Using these deeply and supervisedly learned features has led to a rapid advance in the state-of-the-art for a number of domains \cite{razavian2014cnn}. Our method can be seen as a new approach to training such networks, aimed at improving transfer to new tasks with very small training sets.


%An intelligent agent is one that is able to learn to solve new problems quickly. A good representation of some input domain is one that allows its holder to learn to solve new problems from fewer samples. Constructing representations that allow our learning machinery to generalize accurately to new tasks with just a few samples has the potential to improve performance of machine learning components in low sample settings. Such settings range from using learned features to represent images to improve classification accuracy on a new task (supervised learning), to teaching a robot how to cook from a few demonstrations (reinforcement learning)\footnote{this work will focus solely on the supervised learning variant.}. In such settings, it is better to be able to learn a new function approximator with only a few samples, as in many domains, labeled data is scarce and/or expensive.

%This idea of learning representations that are useful for unseen tasks is certainly not new. It is referred to with multiple names like lifelong learning \cite{thrun1995lifelong}, online multitask learning \cite{saha2011online}, learning to learn \cite{thrun1996learning}, never ending learning \cite{carlson2010toward}, inductive bias learning \cite{baxter2000model}, etc... . The kind of learner we concern our selves with is a persistent agent facing a continuous stream of problems. The agent would ideally be able to use information extracted from past tasks to reduce the amount of information required to generalize well on future tasks. This framework is distinct from multitask learning \cite{caruana1997multitask} in the sense that it focuses on improving generalization performance for new tasks with minimal amounts of training data, rather than focusing on improving generalization performance for a fixed collection of tasks defined a priori. Intuitively, our learner tries to propagate useful information forward in time, from past tasks to future tasks, while a multitask learner tries to share information a-temporally, among a static collection of tasks.


%Most of the algorithms proposed thus far for multitask and lifelong learning, e.g.~\cite{kumar2012learning,baxter2000model,saha2011online,ando2005framework}, rely heavily on a subtle assumption that seems to violate the premises motivating lifelong learning. We call this the assumption of \emph{task correspondence}. To assume task correspondence, our envisioned machine learning service provider, upon being faced with a new task, must have access to a mapping between labels for the new task and labels encountered in previous tasks\footnote{We use ``label'' for categorical and continuous target outputs.}. When such a mapping is available, the service provider can directly transfer label-specific models based on information aggregated over previous tasks to the new task, possibly adapting the transferred models using the labeled data from the new task. For example, in the standard supervised learning setting a labeled set of observations is used to train a model and the trained model is then used to infer labels for new observations. This corresponds to a lifelong learning problem with one past task, defined by the labeled training data, where all labels for future tasks are assumed to be in one-to-one correspondence with the training labels.

%Most algorithms proposed thus far for multitask and lifelong learning, e.g., ~\cite{kumar2012learning,baxter2000model,saha2011online,ando2005framework}, rely on a subtle assumption that seems to violate the premises motivating lifelong learning. We call this the assumption of \emph{task correspondence}. Assuming task correspondence, means our envisioned MLSP has explicit information during either training or testing on which task it is working with. For a concrete example consider the algorithm "Multi-task Feature Learning" \cite{argyriou2007multi}. The algorithm follows an alternating optimization scheme which is common to representation learning approaches to multitask learning. In each step of the optimization, the algorithm optimizes a set of function approximators, one for each task, then it optimizes a shared representation. To be able to do so, the algorithm needs to maintain a number of parameters at least linear in the number of tasks. It also needs to know which parameters to update when seeing each task. While this seems like a reasonable thing to do when the number of tasks is fixed, it is certainly not scalable to the kind of setting we are interested in, where tasks flow in an online manner.

%Our interest in this particular setting comes directly from our MLSP framework. Concretely, imagine an MLSP whose service is face recognition. Clients present the provider with a small set of faces labeled as interesting and not interesting. Clients then request the provider to construct hypotheses that allow them to recognize face images they might find interesting. We can not expect users to enter large amounts of labeled data to solve their tasks, hence the small sample assumption. We assume the number of tasks is too large to be stored, hence the restricted storage assumption. We do not wish to restrict users to a specific set of tasks they can select from, hence we cannot assume task correspondence.

%Another example is one where our MLSP is a website which directs users to available information (e.g.~blog posts, news articles, etc.) based on their observed history of likes/dislikes for information they have already seen. In this case, new users may continually join the site with only a minimal amount of like/dislike information made available a priori, and new information may continually become available. Intuitively, one might assume that there exists some ``coarsest-common-partition (CCP)'' of the set of available information sources such that the users' binary partitions of information space into things they like or dislike can be approximated by binary partitions that do not further divide any elements of the CCP. If our MLSP could learn about the structure of the CCP from the likes and dislikes of its users, then its performance could improve dramatically, by providing better recommendations to existing users and by more rapidly accommodating new users and new information sources.

%In addition to its possible impossibility, the task correspondence assumption may be computationally burdensome to exploit when the number of tasks is exceedingly large. 

%Usually, task correspondence is related to the space consumed by the model: i.e., for the model to be able to remember the tasks it has seen, it has to maintain a data structure that consumes at least linear space in the number of tasks. As this data structure becomes larger, it could consume more time to update, thus incurring a performance penalty in addition to the space penalty as in the model proposed by \cite{kumar2012learning}.

%The penalty incurred by task correspondence is not merely in space and time, but also in applicability, as it limits the performance of a multitask learner in the lifelong learning setting. For instance, one reasonable setting where this correspondence is difficult to obtain in the context of image search is when a service provider with a large number of users allows users the ability to find pictures that contain specific faces in their photo albums. In such a setting, two different users may want to recognize pictures of the same person in their albums. Therefore, the underlying problem they pose is the same and ideally, the classifier provided by the service provider should be the same. However, it is unreasonable to expect these users to present the very same picture of the person they are looking for. It is also unrealistic to assume the learner to be able to compute this correspondence. Another example that illustrates the importance of this scenario is in the context of a website with many users who can "like" certain documents. In this context, it is reasonable to assume that there is an underlying dichotomization according to which users like documents. It is also reasonable to assume that some users have similar tastes, therefore, the underlying problem of classifying articles as of being to these users is identical. However, two users with the same taste may like different articles. Hence task correspondence in this context is not computable without expending effort labelling these documents.

%The setting we propose is thus a truly lifelong learning setting, where the number of tasks is very large and has to be dealt with in an online manner. Also, information about different tasks cannot be stored in a linear fashion and task correspondence is not computable. 







%Our work is also connected to the work of Jonathan Baxter \cite{baxter2000model} in which a formalization of the lifelong learning problem is presented. This work is also related to Baxter's earlier work \cite{baxter1995learning}, in which he proposes the idea of multitask learning with a neural network. Despite being 15 years old, Baxter's works encompass in their generality state-of-the-art models such as deep neural networks. We further elaborate these connections in section 3.

%Structure wise, this paper is divided into five sections. In section 2 we formalize the online multitask learning setting. In section 3, we briefly discuss how our work falls into place given related works in the literature. In section 4, we show how looking at online multitask learning as a representation learning problem leads to an intuitive, efficient algorithm which relies on learning features that are more discriminative than ones learned by standard methods. Finally, in section 5, we present empirical results showing how our algorithm fares as a supervised representation learner, as a multitask learner and as a lifelong learner.

==> chapters/introduction__Ouais_Alsharif_s_conflicted_copy_2014-04-10_.tex <==
%!TEX root = ../ldr.tex

When faced with a new problem, humans can quickly learn to solve that problem with only a few labelled samples. Our intuitive understanding says that humans have a representation of the world that allows this quick generalization. The construction of representations that allow our learning machinery to generalize accurately with just a few samples is crucial to improve performance of machine learning components in various settings. Such settings range from using the learned features to represent images to better classify them (supervised learning), to teaching a robot how to cook from a few demonstrations (reinforcement learning). In such settings, it is always better to be able to learn a new function approximator with only a few samples, as in many domains, labelled data is scarce and/or expensive.

This idea of learning representations that are useful for new tasks is certainly not new. It is referred to with multiple names like lifelong learning \cite{thrun1995lifelong}, online multitask learning \cite{saha2011online}, learning to learn \cite{thrun1996learning}, never ending learning \cite{carlson2010toward}, inductive transfer learning, etc... . The kind of  learner we concern our self with is a persistent agent facing a continuous stream of problems. The agent would ideally be able to use information extracted from past tasks to reduce the amount of information required to generalize well on future tasks. This framework is distinct from multitask learning \cite{caruana1997multitask} in the sense that it focuses on improving generalization performance for new tasks with minimal amounts of training data, rather than focusing on improving generalization performance for a fixed collection of tasks defined a priori. Intuitively, our learner tries to propagate useful information forward in time, from past tasks to future tasks, while a multitask learner tries to share information a-temporally, among a static collection of tasks.

%Most of the algorithms proposed thus far for multitask and lifelong learning, e.g.~\cite{kumar2012learning,baxter2000model,saha2011online,ando2005framework}, rely heavily on a subtle assumption that seems to violate the premises motivating lifelong learning. We call this the assumption of \emph{task correspondence}. To assume task correspondence, our envisioned machine learning service provider, upon being faced with a new task, must have access to a mapping between labels for the new task and labels encountered in previous tasks\footnote{We use ``label'' for categorical and continuous target outputs.}. When such a mapping is available, the service provider can directly transfer label-specific models based on information aggregated over previous tasks to the new task, possibly adapting the transferred models using the labeled data from the new task. For example, in the standard supervised learning setting a labeled set of observations is used to train a model and the trained model is then used to infer labels for new observations. This corresponds to a lifelong learning problem with one past task, defined by the labeled training data, where all labels for future tasks are assumed to be in one-to-one correspondence with the training labels.

Most of the algorithms proposed thus far for multitask and lifelong learning, e.g.~\cite{kumar2012learning,baxter2000model,saha2011online,ando2005framework}, rely heavily on a subtle assumption that seems to violate the premises motivating lifelong learning. We call this the assumption of \emph{task correspondence}. Assuming task correspondence, means iyr envisioned machine learning provider knows during both training and testing which task it is learning. 

have access to a mapping between labels for the new task and labels encountered in previous tasks\footnote{We use ``label'' for categorical and continuous target outputs.}. When such a mapping is available, the service provider can directly transfer label-specific models based on information aggregated over previous tasks to the new task, possibly adapting the transferred models using the labeled data from the new task. For example, in the standard supervised learning setting a labeled set of observations is used to train a model and the trained model is then used to infer labels for new observations. This corresponds to a lifelong learning problem with one past task, defined by the labeled training data, where all labels for future tasks are assumed to be in one-to-one correspondence with the training labels.

Task correspondence is a strong assumption which may be inapplicable in some practical scenarios. For example, imagine a service provider whose service is face recognition. Clients present the provider with a small set of faces labelled as interesting and not interesting. The clients then request the provider to construct a hypothesis that allows them to recognize other face images they might find interesting. In this context, faces that are interesting to one person need not be interesting to another. Hence, task correspondence cannot be assumed. Another example is one where our ML service provider is a website which directs users to available information (e.g.~blog posts, news articles, etc.) based on their observed history of likes/dislikes for information they've already seen. In this case, new users may continually join the site with only a minimal amount of like/dislike information made available a priori, and new information may continually become available. Intuitively, one might assume that there exists some ``coarsest-common-partition (CCP)'' of the set of available information sources such that the users' binary partitions of information space into things they like or dislike can be approximated by binary partitions that don't further divide any elements of the CCP. If our ML service provider could learn about the structure of the CCP from the likes and dislikes of its users, then its performance could improve dramatically, by providing better recommendations to existing users and by more rapidly accommodating new users and new information sources.

%In addition to its possible impossibility, the task correspondence assumption may be computationally burdensome to exploit when the number of tasks is exceedingly large. 

%Usually, task correspondence is related to the space consumed by the model: i.e., for the model to be able to remember the tasks it has seen, it has to maintain a data structure that consumes at least linear space in the number of tasks. As this data structure becomes larger, it could consume more time to update, thus incurring a performance penalty in addition to the space penalty as in the model proposed by \cite{kumar2012learning}.

%The penalty incurred by task correspondence is not merely in space and time, but also in applicability, as it limits the performance of a multitask learner in the lifelong learning setting. For instance, one reasonable setting where this correspondence is difficult to obtain in the context of image search is when a service provider with a large number of users allows users the ability to find pictures that contain specific faces in their photo albums. In such a setting, two different users may want to recognize pictures of the same person in their albums. Therefore, the underlying problem they pose is the same and ideally, the classifier provided by the service provider should be the same. However, it is unreasonable to expect these users to present the very same picture of the person they are looking for. It is also unrealistic to assume the learner to be able to compute this correspondence. Another example that illustrates the importance of this scenario is in the context of a website with many users who can "like" certain documents. In this context, it is reasonable to assume that there is an underlying dichotomization according to which users like documents. It is also reasonable to assume that some users have similar tastes, therefore, the underlying problem of classifying articles as of being to these users is identical. However, two users with the same taste may like different articles. Hence task correspondence in this context is not computable without expending effort labelling these documents.

%The setting we propose is thus a truly lifelong learning setting, where the number of tasks is very large and has to be dealt with in an online manner. Also, information about different tasks cannot be stored in a linear fashion and task correspondence is not computable. 

In this paper, we propose a novel model for lifelong learning which doesn't require information about task correspondence. Our model is motivated by an idea adapted from \cite{baxter2000model}: a lifelong learner should use information from past tasks to learn a representation that is simple enough to allow for effective generalization on new tasks with minimal training data, yet flexible enough to accommodate a relatively diverse set of tasks. In Section 2, we describe the lifelong learning problem more formally and further discuss the benefits of not relying on task correspondence. In Section 3, we briefly discuss some existing approaches to multitask and lifelong learning. In Section 4, we show how looking at lifelong learning as a representation learning problem leads to an intuitive, efficient algorithm which we call Lifelong Learning of Discriminative Representations. Section 5 presents empirical results showing how our algorithm fares in three different contexts: as a supervised representation learner, as a multitask learner, and as a lifelong learner.


==> chapters/introduction__Philip_Bachman_s_conflicted_copy_2014-05-28_.tex <==
%!TEX root = ../ldr.tex
When facing a learning problem with relatively few labelled samples, one has three options:
\begin{enumerate}
\item Use domain knowledge.
\item Use unlabelled samples. 
\item Use labelled samples from a different problem.
\end{enumerate}

The representation learning community has generally focused on the second option. Methods like Deep Boltzmann Machines \cite{salakhutdinov2009deep}, Stacked Denoising Autoencoders \cite{vincent2010stacked}, and Sparse Coding \cite{raina2007self} can be used to learn representations from unlabelled samples. The representations are then either discriminatively fine-tuned via backpropagation, or used as is to extract features for a new problem.

Along related lines, one approach commonly applied to multitask learning is to learn representations that are useful for multiple simultaneous tasks. In multitask learning, a set of tasks is fixed a priori and the learner seeks a model that generalizes well to unseen samples from these tasks. While multitask learning has often facilitated improved generalization to unseen samples, designing learners that can generalize well to unseen tasks has proven more challenging. This latter type of transfer is generally referred to as inductive bias learning \cite{baxter2000model}, lifelong learning \cite{thrun1995lifelong}, learning to learn \cite{thrun1996learning}, or never ending learning \cite{carlson2010toward}, among other names.

Most transfer learning methods concern themselves with situations where data from the target domain is scarce, because when ample data is available in the target domain learning can succeed without drawing on outside information. Interest in such data-scarce regimes is well justified from a practical point of view, as in many situations we are restricted to small amounts of data. Examples of such situations include those in which data is expensive to label (e.g., medical images) and those where it is impractical to obtain large amounts of data (e.g., human computer interaction).

This paper presents a meta-algorithm for online multitask and transfer learning. The intuition we build on is that good representations should allow accurate generalization on new tasks from only a small number of samples. Our method operates on a parametric feature extractor and an algorithm for training function approximators by altering the output of the former to be more effective as input to the latter. It does so by empirically estimating and minimizing the generalization error of function approximators trained on the extracted features, as a function of the feature extractor parameters.

To motivate the particular setting we are concerned with, imagine a Machine Learning Service Provider (MLSP) facing a continuous stream of problems with the same input domain, but with output domains that may differ. Each new problem is presented to the MLSP implicitly through a small batch of labelled examples. For each presented problem the MLSP seeks to learn a new function approximator that generalizes well, i.e.~minimizes test error. To succeed, the MLSP needs a representation of its input domain that permits effective learning from relatively few samples. 

One example of such a MLSP is a website which directs users to available information (e.g.~blog posts, news articles, etc.) based on their observed history of likes/dislikes for information they have already seen. In this case, new users may continually join the site with only a minimal amount of like/dislike information made available a priori, and new information may continually become available. Intuitively, one might assume that there exists some ``coarsest-common-partition'' (CCP) of the set of available information sources such that the users' binary partitions of information space into things they like or dislike can be approximated by binary partitions that do not further divide any elements of the CCP. If our MLSP could learn about the structure of the CCP from the likes and dislikes of its users, its performance would improve dramatically, leading to better recommendations for existing users and more rapid accommodation of new users and information sources.

One major difficulty of learning online from a stream of tasks stems from an inability to store information that identifies each task, as each new task is defined implicitly through the labels provided for it. Moreover, since the number of tasks could be very large, the memory requirements of a practical algorithm should be sublinear in the number of tasks. Algorithms that address this situation seek to minimize error on yet unseen tasks, propagating useful information between tasks forward in time. This is in contrast to standard multitask learning, where the number of tasks is finite and the learner seeks to share information a-temporally, among a static collection of tasks.

%An intelligent agent is one that is able to learn to solve new problems quickly. A good representation of some input domain is one that allows its holder to learn to solve new problems from fewer samples. Constructing representations that allow our learning machinery to generalize accurately to new tasks with just a few samples has the potential to improve performance of machine learning components in low sample settings. Such settings range from using learned features to represent images to improve classification accuracy on a new task (supervised learning), to teaching a robot how to cook from a few demonstrations (reinforcement learning)\footnote{this work will focus solely on the supervised learning variant.}. In such settings, it is better to be able to learn a new function approximator with only a few samples, as in many domains, labelled data is scarce and/or expensive.

%This idea of learning representations that are useful for unseen tasks is certainly not new. It is referred to with multiple names like lifelong learning \cite{thrun1995lifelong}, online multitask learning \cite{saha2011online}, learning to learn \cite{thrun1996learning}, never ending learning \cite{carlson2010toward}, inductive bias learning \cite{baxter2000model}, etc... . The kind of learner we concern our selves with is a persistent agent facing a continuous stream of problems. The agent would ideally be able to use information extracted from past tasks to reduce the amount of information required to generalize well on future tasks. This framework is distinct from multitask learning \cite{caruana1997multitask} in the sense that it focuses on improving generalization performance for new tasks with minimal amounts of training data, rather than focusing on improving generalization performance for a fixed collection of tasks defined a priori. Intuitively, our learner tries to propagate useful information forward in time, from past tasks to future tasks, while a multitask learner tries to share information a-temporally, among a static collection of tasks.


%Most of the algorithms proposed thus far for multitask and lifelong learning, e.g.~\cite{kumar2012learning,baxter2000model,saha2011online,ando2005framework}, rely heavily on a subtle assumption that seems to violate the premises motivating lifelong learning. We call this the assumption of \emph{task correspondence}. To assume task correspondence, our envisioned machine learning service provider, upon being faced with a new task, must have access to a mapping between labels for the new task and labels encountered in previous tasks\footnote{We use ``label'' for categorical and continuous target outputs.}. When such a mapping is available, the service provider can directly transfer label-specific models based on information aggregated over previous tasks to the new task, possibly adapting the transferred models using the labeled data from the new task. For example, in the standard supervised learning setting a labeled set of observations is used to train a model and the trained model is then used to infer labels for new observations. This corresponds to a lifelong learning problem with one past task, defined by the labeled training data, where all labels for future tasks are assumed to be in one-to-one correspondence with the training labels.

%Most algorithms proposed thus far for multitask and lifelong learning, e.g., ~\cite{kumar2012learning,baxter2000model,saha2011online,ando2005framework}, rely on a subtle assumption that seems to violate the premises motivating lifelong learning. We call this the assumption of \emph{task correspondence}. Assuming task correspondence, means our envisioned MLSP has explicit information during either training or testing on which task it is working with. For a concrete example consider the algorithm "Multi-task Feature Learning" \cite{argyriou2007multi}. The algorithm follows an alternating optimization scheme which is common to representation learning approaches to multitask learning. In each step of the optimization, the algorithm optimizes a set of function approximators, one for each task, then it optimizes a shared representation. To be able to do so, the algorithm needs to maintain a number of parameters at least linear in the number of tasks. It also needs to know which parameters to update when seeing each task. While this seems like a reasonable thing to do when the number of tasks is fixed, it is certainly not scalable to the kind of setting we are interested in, where tasks flow in an online manner.

%Our interest in this particular setting comes directly from our MLSP framework. Concretely, imagine an MLSP whose service is face recognition. Clients present the provider with a small set of faces labelled as interesting and not interesting. Clients then request the provider to construct hypotheses that allow them to recognize face images they might find interesting. We can not expect users to enter large amounts of labelled data to solve their tasks, hence the small sample assumption. We assume the number of tasks is too large to be stored, hence the restricted storage assumption. We do not wish to restrict users to a specific set of tasks they can select from, hence we cannot assume task correspondence.

%Another example is one where our MLSP is a website which directs users to available information (e.g.~blog posts, news articles, etc.) based on their observed history of likes/dislikes for information they have already seen. In this case, new users may continually join the site with only a minimal amount of like/dislike information made available a priori, and new information may continually become available. Intuitively, one might assume that there exists some ``coarsest-common-partition (CCP)'' of the set of available information sources such that the users' binary partitions of information space into things they like or dislike can be approximated by binary partitions that do not further divide any elements of the CCP. If our MLSP could learn about the structure of the CCP from the likes and dislikes of its users, then its performance could improve dramatically, by providing better recommendations to existing users and by more rapidly accommodating new users and new information sources.

%In addition to its possible impossibility, the task correspondence assumption may be computationally burdensome to exploit when the number of tasks is exceedingly large. 

%Usually, task correspondence is related to the space consumed by the model: i.e., for the model to be able to remember the tasks it has seen, it has to maintain a data structure that consumes at least linear space in the number of tasks. As this data structure becomes larger, it could consume more time to update, thus incurring a performance penalty in addition to the space penalty as in the model proposed by \cite{kumar2012learning}.

%The penalty incurred by task correspondence is not merely in space and time, but also in applicability, as it limits the performance of a multitask learner in the lifelong learning setting. For instance, one reasonable setting where this correspondence is difficult to obtain in the context of image search is when a service provider with a large number of users allows users the ability to find pictures that contain specific faces in their photo albums. In such a setting, two different users may want to recognize pictures of the same person in their albums. Therefore, the underlying problem they pose is the same and ideally, the classifier provided by the service provider should be the same. However, it is unreasonable to expect these users to present the very same picture of the person they are looking for. It is also unrealistic to assume the learner to be able to compute this correspondence. Another example that illustrates the importance of this scenario is in the context of a website with many users who can "like" certain documents. In this context, it is reasonable to assume that there is an underlying dichotomization according to which users like documents. It is also reasonable to assume that some users have similar tastes, therefore, the underlying problem of classifying articles as of being to these users is identical. However, two users with the same taste may like different articles. Hence task correspondence in this context is not computable without expending effort labelling these documents.

%The setting we propose is thus a truly lifelong learning setting, where the number of tasks is very large and has to be dealt with in an online manner. Also, information about different tasks cannot be stored in a linear fashion and task correspondence is not computable. 

While initially motivated by learning representations for inter-task transfer from large numbers of encountered tasks, the algorithm we propose can also improve transfer to new tasks when learning from just a single encountered task. In that spirit our work is connected to a recent phenomenon in the computer vision community wherein deep neural networks are trained on a single task with many classes and large amounts of labelled data, after which the features learned by the networks are applied to tasks other than the training task, for which few labelled samples are available \cite{razavian2014cnn,Jia13caffe,donahue2013decaf}. Using these deeply and supervisedly learned features has led to a rapid advance in the state-of-the-art for a number of domains \cite{razavian2014cnn}. Our method can be seen as a new approach to training such networks, aimed at improving transfer to new tasks with very few labelled samples.

%Our work is also connected to the work of Jonathan Baxter \cite{baxter2000model} in which a formalization of the lifelong learning problem is presented. This work is also related to Baxter's earlier work \cite{baxter1995learning}, in which he proposes the idea of multitask learning with a neural network. Despite being 15 years old, Baxter's works encompass in their generality state-of-the-art models such as deep neural networks. We further elaborate these connections in section 3.

%Structure wise, this paper is divided into five sections. In section 2 we formalize the online multitask learning setting. In section 3, we briefly discuss how our work falls into place given related works in the literature. In section 4, we show how looking at online multitask learning as a representation learning problem leads to an intuitive, efficient algorithm which relies on learning features that are more discriminative than ones learned by standard methods. Finally, in section 5, we present empirical results showing how our algorithm fares as a supervised representation learner, as a multitask learner and as a lifelong learner.

==> chapters/introduction_ouais.tex <==
%!TEX root = ../ldr.tex

We are constantly facing learning problems for which only few labelled samples exist. Such problems range from those in which data is expensive to label (e.g., medical images) to those where it is practically infeasible to obtain large amounts of labelled data (e.g., human computer interaction).

Generally, when facing such a problem, one has three options: 

\begin{enumerate}
\item Use domain knowledge.
\item Use unlabelled samples.
\item Use labelled samples from a different, but related problem.
\end{enumerate}

Bayesian methods \cite{fei2007learning} extensively explored the first option, relying on knowledge of the target problem's structure to bias search in the target task's hypothesis space. Other methods, like manifold regularization \cite{belkin2006manifold} blend the first and second options, combining both domain knowledge (through a distance metric for instance) and unlabelled samples.

In the representation learning community, more emphasis was placed on learning from unlabelled data with as little domain knowledge as possible. A number of methods like deep Boltzmann machines \cite{salakhutdinov2009deep}, stacked denoising autoencoders \cite{vincent2010stacked} and sparse coding \cite{raina2007self} were shown to be effective for problems with few labelled samples. After training, these representations are either discriminatively fine-tuned via backpropagation, or used as is to extract features for a new problem.

While methods from the two first categories work relatively well for a variety of problems, they ignore the existence of large amounts of labelled data from different, but possibly related problems, which could potentially provide significant gains. The transfer learning community has sought to leverage this idea through a variety of methods grouped under supervised transfer. The most common tools for supervised transfer come from the multitask learning sub-field \cite{caruana1997multitask}, in which a set of tasks is \textit{fixed a priori} and the learner seeks a model that generalizes well to \textit{unseen samples} from these tasks. While multitask learning has been effective in many situations, it falls short in environments where tasks stream sequentially and one seeks to generalize on yet \textit{unseen tasks}. This more challenging type of transfer is generally referred to as inductive bias learning \cite{baxter2000model}, lifelong learning \cite{thrun1995lifelong}, learning to learn \cite{thrun1996learning}, or never ending learning \cite{carlson2010toward}, among other names.

%Most transfer learning methods concern themselves with situations when data on the target domain is scarce. This is because the gain from transfer diminishes as more data is available in the target domain. Interest in such data scarce regimes is well justified from a practical point of view, as in many situations we are restricted to small amounts of data. Examples of such situations include those in which data is expensive to label (e.g, medical images) to those where it is practically infeasible to obtain large amounts (e.g, human computer interaction).

This paper is concerned with learning in such environments, where tasks flow in a sequential manner. To further elucidate the particular setting we are interested in, imagine a Machine Learning Service Provider (MLSP) facing a continuous stream of problems with the same input domain, but with output domains that may differ. Each new problem is presented to the MLSP implicitly through a small batch of labelled examples. For each presented problem the MLSP seeks to learn a new function approximator that generalizes well, i.e.~minimizes test error. To succeed, the MLSP needs a representation of its input domain that permits effective learning from relatively few samples. One example of such MLSP is a website whose service is user-customized face recognition. Clients login continuously to the website. Each client presents the provider with a small set of faces labelled as interesting and not interesting. Then, the client requests the provider to construct a hypothesis that the client can use to detect interesting faces. If the provider has a good representation of the faces space, it should be able to return a good hypothesis function, even if for the new task, only a small amount of labelled data is presented.


%On example of such MLSP is a website which directs users to available information (e.g.~blog posts, news articles, etc.) based on their observed history of likes/dislikes for information they have already seen. In this case, new users may continually join the site with only a minimal amount of like/dislike information made available a priori, and new information may continually become available. Intuitively, one might assume that there exists some ``coarsest-common-partition (CCP)'' of the set of available information sources such that the users' binary partitions of information space into things they like or dislike can be approximated by binary partitions that do not further divide any elements of the CCP. If our MLSP could learn about the structure of the CCP from the likes and dislikes of its users, its performance could improve dramatically. This performance would be depicted by providing better recommendations to existing users and by more rapidly accommodating new users and new information sources.

Our envisioned MLSP faces several difficulties. In terms of scalability, since the number of tasks could be very large, both memory requirements and per-task computational requirements of a practical algorithm should be sublinear in the number of tasks. In terms of usability, since its undesired for the MLSP to constrain its clients to a fixed set of tasks, computation of task relatedness becomes infeasible. This is due to each task being defined implicitly through the labels provided with it. 

While previous works have sought to address similar problems (e.g., \cite{saha2011online, ruvolo2013ella}), the algorithms presented previously suffered from deficiencies in terms of scalability with respect to either the number of tasks or input dimensionality. Experimentally results in previous works were focused on relatively simple multitask learning problems.

In this paper, we present a solution to the problem above that is efficient in \textit{both} input dimensionality and the number of tasks. The intuition we build on is that good representations should allow accurate generalization on new tasks from only a small number of samples. Our method operates on a parametric feature extractor and an algorithm for training differentiable function approximators by altering the output of the former to be more effective as input to the latter. It does so by empirically estimating and minimizing the generalization error of function approximators trained on the extracted features, as a function of the feature extractor parameters.

While initially motivated by learning representations for inter-task transfer from a long stream of tasks, the algorithm we propose can also improve transfer to new tasks when learning from just a single encountered task. In that spirit our work is connected to a recent phenomenon in the computer vision community wherein deep neural networks are trained on a single task with many classes and large amounts of labelled data, after which the features learned by the networks are applied to tasks other than the training task, for which few labelled samples are available \cite{razavian2014cnn,Jia13caffe,donahue2013decaf}. Using these deeply and supervisedly learned features has led to a rapid advance in the state-of-the-art for a number of domains \cite{razavian2014cnn}. Our method can be seen as a new approach to training such networks, aimed at improving transfer to new tasks with very few labelled samples.


%An intelligent agent is one that is able to learn to solve new problems quickly. A good representation of some input domain is one that allows its holder to learn to solve new problems from fewer samples. Constructing representations that allow our learning machinery to generalize accurately to new tasks with just a few samples has the potential to improve performance of machine learning components in low sample settings. Such settings range from using learned features to represent images to improve classification accuracy on a new task (supervised learning), to teaching a robot how to cook from a few demonstrations (reinforcement learning)\footnote{this work will focus solely on the supervised learning variant.}. In such settings, it is better to be able to learn a new function approximator with only a few samples, as in many domains, labelled data is scarce and/or expensive.

%This idea of learning representations that are useful for unseen tasks is certainly not new. It is referred to with multiple names like lifelong learning \cite{thrun1995lifelong}, online multitask learning \cite{saha2011online}, learning to learn \cite{thrun1996learning}, never ending learning \cite{carlson2010toward}, inductive bias learning \cite{baxter2000model}, etc... . The kind of learner we concern our selves with is a persistent agent facing a continuous stream of problems. The agent would ideally be able to use information extracted from past tasks to reduce the amount of information required to generalize well on future tasks. This framework is distinct from multitask learning \cite{caruana1997multitask} in the sense that it focuses on improving generalization performance for new tasks with minimal amounts of training data, rather than focusing on improving generalization performance for a fixed collection of tasks defined a priori. Intuitively, our learner tries to propagate useful information forward in time, from past tasks to future tasks, while a multitask learner tries to share information a-temporally, among a static collection of tasks.


%Most of the algorithms proposed thus far for multitask and lifelong learning, e.g.~\cite{kumar2012learning,baxter2000model,saha2011online,ando2005framework}, rely heavily on a subtle assumption that seems to violate the premises motivating lifelong learning. We call this the assumption of \emph{task correspondence}. To assume task correspondence, our envisioned machine learning service provider, upon being faced with a new task, must have access to a mapping between labels for the new task and labels encountered in previous tasks\footnote{We use ``label'' for categorical and continuous target outputs.}. When such a mapping is available, the service provider can directly transfer label-specific models based on information aggregated over previous tasks to the new task, possibly adapting the transferred models using the labeled data from the new task. For example, in the standard supervised learning setting a labeled set of observations is used to train a model and the trained model is then used to infer labels for new observations. This corresponds to a lifelong learning problem with one past task, defined by the labeled training data, where all labels for future tasks are assumed to be in one-to-one correspondence with the training labels.

%Most algorithms proposed thus far for multitask and lifelong learning, e.g., ~\cite{kumar2012learning,baxter2000model,saha2011online,ando2005framework}, rely on a subtle assumption that seems to violate the premises motivating lifelong learning. We call this the assumption of \emph{task correspondence}. Assuming task correspondence, means our envisioned MLSP has explicit information during either training or testing on which task it is working with. For a concrete example consider the algorithm "Multi-task Feature Learning" \cite{argyriou2007multi}. The algorithm follows an alternating optimization scheme which is common to representation learning approaches to multitask learning. In each step of the optimization, the algorithm optimizes a set of function approximators, one for each task, then it optimizes a shared representation. To be able to do so, the algorithm needs to maintain a number of parameters at least linear in the number of tasks. It also needs to know which parameters to update when seeing each task. While this seems like a reasonable thing to do when the number of tasks is fixed, it is certainly not scalable to the kind of setting we are interested in, where tasks flow in an online manner.

%Our interest in this particular setting comes directly from our MLSP framework. Concretely, imagine an MLSP whose service is face recognition. Clients present the provider with a small set of faces labelled as interesting and not interesting. Clients then request the provider to construct hypotheses that allow them to recognize face images they might find interesting. We can not expect users to enter large amounts of labelled data to solve their tasks, hence the small sample assumption. We assume the number of tasks is too large to be stored, hence the restricted storage assumption. We do not wish to restrict users to a specific set of tasks they can select from, hence we cannot assume task correspondence.

%Another example is one where our MLSP is a website which directs users to available information (e.g.~blog posts, news articles, etc.) based on their observed history of likes/dislikes for information they have already seen. In this case, new users may continually join the site with only a minimal amount of like/dislike information made available a priori, and new information may continually become available. Intuitively, one might assume that there exists some ``coarsest-common-partition (CCP)'' of the set of available information sources such that the users' binary partitions of information space into things they like or dislike can be approximated by binary partitions that do not further divide any elements of the CCP. If our MLSP could learn about the structure of the CCP from the likes and dislikes of its users, then its performance could improve dramatically, by providing better recommendations to existing users and by more rapidly accommodating new users and new information sources.

%In addition to its possible impossibility, the task correspondence assumption may be computationally burdensome to exploit when the number of tasks is exceedingly large. 

%Usually, task correspondence is related to the space consumed by the model: i.e., for the model to be able to remember the tasks it has seen, it has to maintain a data structure that consumes at least linear space in the number of tasks. As this data structure becomes larger, it could consume more time to update, thus incurring a performance penalty in addition to the space penalty as in the model proposed by \cite{kumar2012learning}.

%The penalty incurred by task correspondence is not merely in space and time, but also in applicability, as it limits the performance of a multitask learner in the lifelong learning setting. For instance, one reasonable setting where this correspondence is difficult to obtain in the context of image search is when a service provider with a large number of users allows users the ability to find pictures that contain specific faces in their photo albums. In such a setting, two different users may want to recognize pictures of the same person in their albums. Therefore, the underlying problem they pose is the same and ideally, the classifier provided by the service provider should be the same. However, it is unreasonable to expect these users to present the very same picture of the person they are looking for. It is also unrealistic to assume the learner to be able to compute this correspondence. Another example that illustrates the importance of this scenario is in the context of a website with many users who can "like" certain documents. In this context, it is reasonable to assume that there is an underlying dichotomization according to which users like documents. It is also reasonable to assume that some users have similar tastes, therefore, the underlying problem of classifying articles as of being to these users is identical. However, two users with the same taste may like different articles. Hence task correspondence in this context is not computable without expending effort labelling these documents.

%The setting we propose is thus a truly lifelong learning setting, where the number of tasks is very large and has to be dealt with in an online manner. Also, information about different tasks cannot be stored in a linear fashion and task correspondence is not computable. 







%Our work is also connected to the work of Jonathan Baxter \cite{baxter2000model} in which a formalization of the lifelong learning problem is presented. This work is also related to Baxter's earlier work \cite{baxter1995learning}, in which he proposes the idea of multitask learning with a neural network. Despite being 15 years old, Baxter's works encompass in their generality state-of-the-art models such as deep neural networks. We further elaborate these connections in section 3.

%Structure wise, this paper is divided into five sections. In section 2 we formalize the online multitask learning setting. In section 3, we briefly discuss how our work falls into place given related works in the literature. In section 4, we show how looking at online multitask learning as a representation learning problem leads to an intuitive, efficient algorithm which relies on learning features that are more discriminative than ones learned by standard methods. Finally, in section 5, we present empirical results showing how our algorithm fares as a supervised representation learner, as a multitask learner and as a lifelong learner.

==> chapters/method.tex <==
%!TEX root = ../ldr.tex

We now present the method we propose for addressing the objective in \eqref{ll_obj1}. Our method has the following key properties:
\begin{enumerate}
\item \textbf{Flexibility}: our method is modular, easily accommodating different feature extractors and function approximators.
\item \textbf{Online}: tasks can be presented to our method sequentially and need not be remembered in perpetuity.
\item \textbf{Scalability}: our method scales well with respect to: the number of samples per task, the number of tasks, the dimension of the input domain, and the dimension of the extracted-feature domain.
%\item \textbf{Task Correspondence}: is not required by our model.
\end{enumerate} 

The general idea of our model is to wrap a parametric feature extractor $f$ and an unbounded collection of trainable function approximators $\{...,h_i,...\}$ with a ``meta'' algorithm that tries to make the output of $f$ more effective as input to the algorithm $\AAA_i$ used to train $h_i$ for task $\TT_i$\footnote{The collection of function approximators may be unbounded, but we select each algorithm/approximator pair $\AAA_i/h_i$ from a finite set of methods, e.g.,~linear logistic regression for classification tasks and linear least-squares regression for regression tasks.}. Using the notation defined in Section 2, our objective is given by:
\begin{equation}
\minimize_{\theta \in \Theta} \mathbb{E}_{\TT_i \sim \QQ} \mathbb{E}_{(X_i^m, Y_i^m) \sim \DD_i} \GG_i \left( \AAA_i(f_{\theta}(X_i^m), Y_i^m) \right),
\label{ldr_obj_true}
\end{equation}
where $f_{\theta}$ represents setting the parameters of the parametric function approximator $f$ to $\theta$. This objective is an instance of the objective in \eqref{ll_obj1} in which the structure sharing among the per-task algorithms, i.e.,~the $\AAA_i^{\theta}$ in \eqref{ll_obj1}, is effected by using the same parameterized feature extractor $f_{\theta}$ to preprocess inputs to each $\AAA_i$.

The particular novelty in our method is that we explicitly minimize an empirical proxy for the expected per-task small-sample generalization errors given by $\GG_i \left( \AAA_i(f(X_i^m), Y_i^m) \right)$. In contrast, typical approaches to multitask learning simultaneously learn a feature extractor $f_{\theta}$ and a collection of task-adapted functions $\hat{h}_i$ for a fixed set of tasks $\{\TT_1,...,\TT_n\}$. This approach seeks an $f$ such that there exist functions $\hat{h}_i$ with small error, w.r.t.~$\LL_i^{\AAA}$, on the training sets available for each $\TT_i$. 


%In particular, these approaches do not explicitly account for the small-sample learnability of the functions $\hat{h}_i$\footnote{Here, learnability roughly means the probability that algorithm $\AAA_i$ finds $\hat{h}_i \in \HH_i^{\AAA}$ with small $\GG_i(\hat{h}_i)$ given the small $m$-sample $(f(X_i^m), Y_i^m)$ used in the search over $\HH_i^{\AAA}$.}. 

%This shift in perspective informs the structure of our method and produces improved empirical performance in practically-relevant scenarios.

\begin{figure}
  \centering
  \includegraphics[scale=.7]{materials/drawing.pdf}
  \caption{Discriminative Representations for Online Transfer}
\end{figure}

Given $T$ $m$-samples $\{(X_1^m, Y_1^m),...,(X_T^m,Y_T^m)\}$ drawn from its environment, our algorithm optimizes the following empirical approximation of \eqref{ldr_obj_true}:
\begin{equation}
\minimize_{\theta \in \Theta} \frac{1}{T} \sum_{i=1}^{T} \hat{\GG}_i(\AAA_i, (f_{\theta}(X_i^m), Y_i^m)),
\end{equation}
where $\hat{\GG}_i$ is an empirical estimate of generalization functional on task $i$. To define $\hat{\GG}_i$, we first define a process for sampling a pseudo-training/validation set pair $(tr_i^n, va_i^{m-n})$ from the $m$-sample $(X_i^m, Y_i^m)$ available for $\TT_i$. We sample the pseudo-train/validate split $(tr_i^n, va_i^{m-n})$ by randomly sampling $n < m$ observations $(x_i,y_i)$ for $tr_i^n$, from $(X_i^m, Y_i^m)$, and then let $va_i^{m-n}$ contain the remaining $m - n$ observations in $(X_i^m, Y_i^m)$.
Now, we compute $\hat{\GG}_i$ as follows:
\begin{align*}
\hat{\GG}_i(\AAA_i, (f_{\theta}(X_i^m, Y_i^m))) =
\mathbb{E}_{(tr_i^n, va_i) \sim (X_i^m, Y_i^m)} \left[ \sum_{(x_j, y_j) \in va_i} \LL_i^{\AAA}(\hat{h}_i^n(f_{\theta}(x_j)), y_j) \right],
\end{align*}
in which $\hat{h}_i^n = \AAA_i(tr_i^n)$ indicates the hypothesis produced by applying algorithm $\AAA_i$ to the pseudo-training set $tr_i^n$. 

%When the number of available tasks is small, we approximate sampling a random task $\TT_i$ from $\QQ$ by sampling $\TT_i$ at random from the fixed set of available tasks.

Algorithm \ref{alg:algorithm_1} describes concretely the steps of our algorithm. Figure 1 presents a visual depiction of each step to further elucidate the algorithm. Note that in the loop on line 6, after altering the representation once, the optimal function approximator given the new representation changes. For computational purposes, we approximate the new optimal function with the one acquired before updating the representation.

\begin{algorithm}[tb]
   \caption{Discriminative Representations for Online Transfer}
   \label{alg:algorithm_1}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} Source environment $\EE = (\XX, \QQ)$, pseudo-training batch size $n$, updates per task sample $K$, learning rate $\gamma$.
   \WHILE{ true } 
   \STATE Sample task $\TT_i \sim \QQ$, with $m$-sample $(X_i^m,Y_i^m)$
   \STATE Sample train/validate split $(tr_i^n, va_i^{m-n}) \sim (X_i^m,Y_i^m)$
   \STATE Apply $\AAA_i$ to $tr_i^n$ to get $\hat{h}_i^n$.
   \FOR{$k=1$ {\bfseries to} $K$}   
	   \STATE Sample a minibatch $\tilde{va}_i^n$ from $va_i^n$.
	   \STATE Define $(\tilde{X}, \tilde{Y})$ such that $\tilde{va}_i^n = (\tilde{X}, \tilde{Y})$.
	   \STATE Let $\theta := \theta - \gamma \nabla_{\theta} \LL_i^{\AAA}(\hat{h}_i^n(f_{\theta}(\tilde{X})), \tilde{Y})$
   \ENDFOR
   \ENDWHILE
   
\end{algorithmic}
\end{algorithm}


==> chapters/method__Ouais_Alsharif_s_conflicted_copy_2014-02-04_.tex <==
%!TEX root = ../ldr.tex

We now present the model we propose for addressing the optimization in \eqref{ll_obj1}, which has the following key properties:
\begin{enumerate}
\item \textbf{Flexibility}: our model is modular, easily accommodating different feature extractors and function approximators.
\item \textbf{Online}: tasks can be presented to our model sequentially and need not be remembered in perpetuity.
\item \textbf{Scalability}: our model scales well with respect to: the number of samples per task, the number of tasks, the dimension of the input domain, and the dimension of the extracted-feature domain.
\item \textbf{Task Correspondence}: our model does not require it.
\end{enumerate} 
The general idea of our model is to wrap a trainable feature extractor $f_{\theta}$ and an unbounded collection of trainable function approximators $\{...,h_t,...\}$ with a ``meta'' algorithm that tries to make the output of the feature extractor more effective as input to the algorithm $\AAA_t$ used to train function approximator $h_t$ for task $\TT_t$\footnote{The collection of function approximators may be unbounded, but we select each algorithm/approximator pair $\AAA_t/h_t$ from a finite pool of methods, e.g.~linear logistic regression for classification tasks and linear least-squares regression for regression tasks.}. Using the notation defined in Section 2, our objective is given by:
\begin{equation}
\minimize_{\theta \in \Theta} \mathbb{E}_{\TT_t \sim \QQ} \mathbb{E}_{(X_t^m, Y_t^m) \sim \DD_t} \GG_t \left( \AAA_t(f_{\theta}(X_t^m), Y_t^m) \right),
\end{equation}
where $f_{\theta}$ represents setting the parameters of the parametric function approximator $f$ to $\theta$.

Where our method differs from existing methods is that we explicitly minimize an empirical proxy for the expected per-task small-sample generalization errors given by $\GG_t \left( \AAA_t(f(X_t^m), Y_t^m) \right)$. In contrast, typical approaches to multitask learning simultaneously learn a feature extractor $f$ and a collection of task-adapted functions $\hat{h}_i$ for a fixed set of tasks $\{\TT_1,...,\TT_n\}$. This approach seeks an $f$ such that there exist functions $\hat{h}_i$ with small error, w.r.t.~$\LL_i^{\AAA}$, on the training sets available for each $\TT_i $. In particular, these approaches do not explicitly account for the small-sample learnability of the functions $\hat{h}_i$\footnote{Here, learnability roughly means the probability that algorithm $\AAA_i$ finds $\hat{h}_i \in \HH_i^{\AAA}$ with small $\GG_i(\hat{h}_i)$ given the small $m$-sample $(f(X_i^m), Y_i^m)$ used in the search over $\HH_i^{\AAA}$.}. This shift in perspective informs the structure of the specific method we present in this work, which produces improved empirical performance in practically-relevant scenarios.

Formally, the objective function we seek to optimize is:
\begin{align}
err = \sum_{i=1}^n \min_h \sum_{j=1}^m L_{\mathcal{T}_i}(h \circ f(x_j), y_j))
\end{align}

To do so, we use an alternating optimization scheme. In which we start by sampling a task: $$\mathcal{T}_i \sim D_\mathcal{Q}$$ 
then we sample a batch of training data from $D_{\mathcal{T}_i}$
$$\{(x_j^{\mathcal{T}_i},y_j^{\mathcal{T}_i})\}_{j=1}^{B_{train}} \sim D_{\mathcal{T}_i}$$
After which we optimize $h$ with $f$ held fixed as follows:

\begin{equation}\label{eq:optimize_h}
\min_h \sum_{j=1}^{B_{train}} L_{\mathcal{T}_i} (h \circ f(x_j),y_j)
\end{equation}

We then sample $K$ batches of size $B_{test}$ each and train $f$ with $h$ held fixed for a single iteration per batch. To be able to do this we need the losses $L_{\mathcal{T}}$ to be differentiable with respect to the parameters of  $h$ so we could "backpropagate" the errors to train $f$. Algorithm 1 depicts our proposed algorithm.

\begin{algorithm}[tb]
   \caption{Discriminative Representation Learner}
   \label{alg:example}
\begin{algorithmic}
   \STATE {\bfseries Input:} task data $D_t$, training batch size $B_{train}$, validation batch size $B_{valid}$, max iterations $N$, iterations per task sample $K$, task distribution $\mathcal{Q}$
   
   \FOR{$i=1$ {\bfseries to} $N$} 
   \STATE Sample task $\mathcal{T} \sim D_\mathcal{Q}$
   \STATE Sample $(X,y)_{B_{train}} \sim D_\mathcal{T}$
   
   \STATE Solve Equation \eqref{eq:optimize_h}
   
   \FOR{$k=1$ {\bfseries to} $K$}   
	   \STATE Sample $(X,y)_{B_{valid}} \sim D_\mathcal{T}$
	   \STATE Update $f$ with $h$ fixed
      
   \ENDFOR
   \ENDFOR
   
\end{algorithmic}
\end{algorithm}

In practice, since we can't sample from $\mathcal{Q}$ nor from $D_{\mathcal{T}_i}$ we consider all the tasks to be of equal probability and we while drawing samples from the set $\{(x_j^{\mathcal{T}_i},y_j^{\mathcal{T}_i})\}_{j=1}^m$ we partition the set into two sets, from the first we sample the training samples and from the second we sample the $K$ batches we use as a proxy for the generalization performance.


==> chapters/problem_definition.tex <==
%TEX root=../ldr.tex
Let our MLSP operate in an environment $\EE = (\QQ, \XX)$, which comprises an input domain $\XX$ and a task distribution $\QQ$. $\QQ$ is a distribution over i.i.d tasks $\TT_i$, where each task $\TT_i = (\YY_i, \DD_i, \LL_i, \GG_i)$ comprises:
\begin{itemize}
\item An output domain $\YY_i$.
\item A distribution $\DD_i$ over $\XX \times \YY_i$.
\item A non-negative loss function $\LL_i: \YY_i \times \YY_i \rightarrow \mathbb{R}^{+}$.
\item A generalization functional $\GG_i(f)$, for all functions $f: \XX \rightarrow \YY_i$, with  $\GG_i(f) = \mathbb{E}_{(x,y) \sim \DD_i} \LL_i(f(x), y)$.
\end{itemize}
For the environments we consider, $\XX = \mathbb{R}^d$. For classification tasks, $\YY_i$ is the discrete space of relevant labels and for regression tasks, $\YY_i = \mathbb{R}$. For classification tasks, the generalization functional $\GG_i(f)$ gives the expected misclassification rate of the classifier $f$ w.r.t.~$\DD_i$. For regression tasks, the generalization functional $\GG_i(f)$ gives the expected error of the regressor $f$, w.r.t.~$\DD_i$. We don't restrict our definitions to specific loss functions as our model is able to accommodate different loss functions (e.g., logistic, ranking, RMSE, etc). 

Loosely speaking, our MLSP is a persistent machine learning agent faced with an environment $\EE$ and tasked with producing hypotheses $\hat{h}_i: \XX \rightarrow \YY_i$ for any tasks $\TT_i$ it encounters, so as to minimize $\mathbb{E}_{\TT_i \sim \QQ} \GG_i(\hat{h}_i)$. To produce a hypothesis $\hat{h}_i$ for task $\TT_i$, the agent first receives an $m$-sample $(X_i^m, Y_i^m) = \{(x_j, y_j)\}_{j=1}^m$ of training observations drawn from $\DD_i$. The agent then applies an algorithm $\AAA_i$ to the $m$-sample to produce a hypothesis $\hat{h}_i$ that minimizes a structured risk. We denote this process as $\hat{h}_i = \AAA_i(X_i^m, Y_i^m)$ and:
\begin{align*}
&\AAA_i(X_i^m, Y_i^m) = \\
&\argmin_{h \in \HH_i^{\AAA}} \frac{1}{m} \sum_{(x_j,y_j) \in (X_i^m, Y_i^m)} \LL_i(h(x_j), y_j) + \RR_i(h),
\end{align*}

where $\HH_i^{\AAA}$ gives the hypothesis space searched by $\AAA_i$, $\LL_i$ gives the loss function minimized by $\AAA_i$, and $\RR_i$ gives any regularization terms used by $\AAA_i$ to bias the search over $\HH_i^{\AAA}$. We let $\AAA_i$ minimize a surrogate loss $\LL_i^{\AAA}$, as the natural task loss $\LL_i$ may provide an intractable optimization objective. In general, the algorithm $\AAA$ is parameterized by some learnable parameters $\theta \in \Theta$ that are meant to capture the shared structure between different tasks. We denote this parameterization as $\AAA^\theta$.

Using the definitions presented thus far, the online transfer learning objective we consider can be written as:

\begin{equation}
\minimize_{\theta \in \Theta} \mathbb{E}_{\TT_i \sim \QQ} \mathbb{E}_{(X_i^m, Y_i^m) \sim \DD_i} \GG_i(\AAA_i^{\theta}(X_i^m, Y_i^m)),\footnote{While we always use $m$ for the number of samples available as input to each $\AAA_i$, in practice $m$ may differ across tasks.} 
\label{ll_obj1}
\end{equation}

Sections 4 and 5 will give more detail on how one might define useful structures to be shared among the per-task estimation problems. Loosely speaking, the objective in~\eqref{ll_obj1} measures the ability of the structurally-biased per-task algorithms $\AAA_i^{\theta}$ to find hypotheses $\hat{h}_i = \AAA_i^{\theta}(X_i^m, Y_i^m)$ that generalize well w.r.t.~$\GG_i$, in a small-sample setting.

==> chapters/related_works.tex <==
%!TEX root = ../ldr.tex
In this section, we present how our work relates to relevant works in the literature. It is important to note, that since this paper touches on multiple sub-fields with extensive works in each, any list we provide will be necessarily incomplete. Since we focus on transfer from labelled data, we will focus here on literature related to supervised transfer. For a more extensive survey on transfer learning consult \cite{pan2010survey}.

Ideas grouped under supervised transfer can be loosely categorized into three sub-fields, namely: ``multitask learning'', ``transductive learning'' and ``lifelong learning''. In multitask learning \cite{caruana1997multitask}, the goal is to solve a number of fixed problems simultaneously, with the hope that by sharing information between tasks, we would achieve better solutions for the problems considered. Many structures have been investigated to share information across tasks, including neural networks \cite{baxter1995learning,caruana1997multitask}, distance metrics \cite{thrun1996learning}, Bayesian priors \cite{xue2007multi}, sparse code dictionaries \cite{kumar2012learning} and others. Overall, multitask learning assumes the marginal distributions of samples seen during testing to be the same as those during training and that with each sample, a specific task id is given.

In transductive learning \cite{daume2006domain,zadrozny2004learning} the source and target tasks are also the same, however the marginal distributions differ between the training and testing samples. The focus of transductive learning has been on correcting for this difference, to improve performance in target domains.

Lifelong learning \cite{baxter2000model,thrun1995lifelong,baxter1995learning} differs from the previous two sub-fields in that target problems are assumed to be \text{distinct} from training problems. Hence, methods used for lifelong learning can be applied in situations where multitask or transductive learning are used. In particular lifelong learning relaxes the task correspondence assumption made by multitask learning. 

Theoretical foundations for lifelong learning were established by \cite{baxter2000model}, wherein PAC bounds for a setting very similar to the one described in section 2 were presented. Though motivated by lifelong learning, the algorithm presented in \cite{baxter2000model} solves a multitask learning problem using a two-part model. The approach they use is the standard approach for multitask learning with neural networks, which extends in its generality to deep models as in \cite{collobert2008unified}.

On the applied side, few works have focused on creating scalable multitask and lifelong learners. One work is that of \cite{saha2011online}, wherein a method for online multitask learning, called OMTL, is proposed\footnote{The word ``online'' in OMTL refers to samples from fixed tasks arriving in an online manner. This environment is distinct from the one faced by our MLSP.}. While OMTL is efficient when the number of tasks is fairly small, it doesn't scale to environments with large number of tasks. This is due to the algorithm maintaining a $T \times T$ task-relatedness matrix when presented with $T$ tasks. Also, its use of a perceptron algorithm as a building block restricts its applicability to classification tasks.

%For OMTL, the target tasks are limited to classification tasks. In terms of scalability, since OMTL targets multitask learning, it does not scale well as the number of tasks increases.  Also, as pointed out by \cite{ruvolo2013ella}, the perceptron algorithm tends to underperform other linear methods (e.g., logistic regression).

%In \cite{saha2011online}, the authors propose a method for multitask learning, called ``Online Multitask Learning'' (OMTL) \footnote{The word ``online'' in OMTL refers to samples from fixed tasks arriving in an online manner. This environment is distinct from the one faced by our MLSP.} based on the perceptron algorithm. For OMTL, the target tasks are limited to classification tasks. In terms of scalability, since OMTL targets multitask learning, it does not scale well as the number of tasks increases. This is due to the algorithm maintaining a $T \times T$ task-relatedness matrix when presented with $T$ tasks. Also, as pointed out by \cite{ruvolo2013ella}, the perceptron algorithm tends to underperform other linear methods (e.g., logistic regression).


%. The reason for that, is the existence of task specific structure that is only updated when that particular task is observed. For a concrete example consider the algorithm ``Multi-task Feature Learning'' \cite{argyriou2007multi}. The algorithm follows an alternating optimization scheme which is common to representation learning approaches to multitask learning. In each step of the optimization, the algorithm optimizes a set of function approximators, one for each task, then it optimizes a shared representation. To be able to do so, the algorithm needs to maintain a number of parameters at least linear in the number of tasks. It also needs to know which parameters to update when seeing each task. While this is reasonable when the number of tasks is finite, it is inapplicable in situations like the one faced by our MLSP.

In seeking to address the inefficiency of multitask learning algorithms in environments with large number of tasks, \cite{ruvolo2013ella} presented an algorithm that builds on a class of methods in multitask learning, in which multiple tasks share a common basis. Their algorithm, ELLA, relies on representing the parameters of the predictive function $f_w$ for a new task using a sparse code over dictionary elements, i.e.~$f_w(x) = (L s)^{\top} x$, where $||s||_1$ is small and $w = L s$. While ELLA is a lifelong learner, consuming $O(T)$ time and $O(1)$ space when observing $T$ tasks, it is inefficient in highly dimensional environments. ELLA is also inefficient when the size of the basis required to represent the data grows. These inefficiencies are due to ELLA's per-task update step, in which the algorithm pays $O(d^3k^2)$ in computation, where $d$ is the dimensionality of the data and $k$ is the number of bases. In addition to these inefficiencies, the linearity of the predictor $f_w$ assumed by ELLA, limits the space of tasks where ELLA might perform well to tasks on which a linear approximator could conceivably perform well given enough training observations.

\begin{table}
\centering
\begin{tabular}{l|c|c|c|c|c}	
    \textbf{Criterion}        & \textbf{OMTL} & \textbf{GOMTL} & \centering \textbf{ELLA}  & \textbf{Our method} & \textbf{Baxter} \\ \hline
	 Online & $\star$   &  & $\star$ &  $\star$ &            \\
     Computation per task & $O(T^2)$& N/A & $O(1)$ & $O(1)$ & $O(1)$ \\
     Space per $T$ tasks & $O(T^2)$ &$O(T)$ & $O(1)$ & $O(1)$ & $O(T)$       \\
     Non-linear $ $ & & & & $\star $ & $\star$
    \end{tabular}
\end{table}
 
% Additionally, the linearity of $f_w$ assumed by ELLA, as presented in \cite{ruvolo2013ella}, limits the space of tasks where ELLA might perform well to tasks on which a linear approximator could conceivably perform well given enough training observations.

%ELLA is similar in structure to another method, called Sparse Coding Multitask  Learner (SCMTL) which encodes the shared structure as a dictionary. In SCMTL, the prediction is the dot product of a data point and a sparse combination of dictionary vectors. SCMTL is easily extendable to RKHS variants via the kernel trick. However **add negatives, maybe after experiments?***




%Many structures through which information is shared have been investigated by previous works, including neural network-based feature transformations \cite{Baxter95learninginternal}, learned distance metrics \cite{thrun1996learning}, Bayesian priors \cite{xue2007multi}, among others.


%The key motivation for lifelong learning is the idea that information extracted from past tasks may be used to improve the $\hat{h}_i$ estimated for future tasks. A similar motivation (adapted for an a-temporal setting) motivates most work on multitask learning. Lifelong learning has deep connections with multitask learning, and can be seen as an online form of multitask learning where the goal is to generalize to new samples \emph{and} new tasks, not just to new samples within existing tasks. In the particular taxonomy of \cite{pan2010survey}, lifelong learning would be classified as inductive multitask learning. In \cite{thrun1996discovering}, the authors provide a listing of early multitask and lifelong learning methods. The listed methods all rely on some structure through which information is shared among tasks. The ubiquity of the shared-structure approach continues through to the present-day. The various structures used to induce information sharing include neural network-based feature transformations \cite{Baxter95learninginternal}, learned distance metrics \cite{thrun1996learning}, Bayesian priors \cite{xue2007multi}, and many others. For a recent survey on transfer learning in general and multitask learning in particular, consulte \cite{pan2010survey}.

%Some recent work has focused on creating efficient, online multitask learners. In particular, \cite{ruvolo2013ella} presents an algorithm for online multitask learning composed of two parts: a linear function approximator $f_{w}(x) = w^{\top} x$ where $w \in \mathbb{R}^d$, and a dictionary $L \in \mathbb{R}^{d \times k}$ containing $k$ $d$-dimensional basis functions. Their algorithm, ELLA, relies on representing the parameters of $f_w$ for a new task using a sparse code over the dictionary elements, i.e.~$f_w(x) = (L s)^{\top} x$, where $||s||_1$ is small and we assume $w = L s$. ELLA was constructed such that it scales well with the number of tasks, therefore satisfying one aspect of the framework we are interested in. However, unfortunately, it doesn't scale well as the dimensionality of the data increases. This results from the way ELLA updates the dictionary $L$ after seeing each new task, which costs $O(d^3k^2)$, where $d$ is the dimensionality of the data and $k$ is the number of basis. Additionally, the linearity of $f_w$ assumed by ELLA, as presented in \cite{ruvolo2013ella}, limits the space of tasks where ELLA might perform well to tasks on which a linear approximator could conceivably perform well given enough training observations.



Among the algorithms surveyed above, only ELLA \cite{ruvolo2013ella} can operate without the task correspondence assumption or alternatively, with a number of parameters sublinear in the number of tasks.



%comprising a trainable feature extractor $f_{\theta}$, parameterized by $\theta \in \Theta$, shared by all tasks and $T$ trainable task-specific function approximators $\{h_1,...,h_T\}$. These function approximators receive the output of $f_{\theta}$ as their inputs. Given an $m$-sample $(X_t^m, Y_t^m)$ for each task, the objective used by Baxter's approach can be written in our notation as:
%\begin{equation}
%\minimize_{\theta \in \Theta, \, \{h_1,...h_T\}} \sum_{t=1}^{T} \sum_{i=1}^{m} \LL_t^{\AAA}(h_t(f_\theta(x_i)), y_i),\label{eq:2}
%\end{equation}
%in which $\LL_t^{\AAA}$ gives the surrogate loss function chosen for each task, to serve as an optimization-friendly proxy for $\LL_t$.

%When Baxter instantiated his work, he used a neural network for the representation $f_{\theta}$ and linear approximators for the per-task function approximators $h_t$. It is crucial to note that Baxter's original formulation of multitask learning with a neural network, despite being almost 20 years old, extends to include state-of-the-art methods like multitask learning with deep neural networks as in \cite{collobert2008unified} and the winning entry in the Merck Molecular Activity Challenge in 2012.

%It is of historical interest to note that Baxter hadn't set out originally to optimize the multitask learning loss \eqref{eq:2}. Rather, the PAC bounds he established are for the objective function:
%\begin{equation}
%\minimize_{\theta \in \Theta} \sum_{t=1}^{T} \minimize_{h_t} \sum_{i=1}^{m} \LL_t^{\AAA}(h_t(f_\theta(x_i)), y_i)\label{eq:3}
%\end{equation}

%which minimizes the generalization error on a new task. Our work bridges this gap, by optimizing the true objective Baxter had set out to optimize. As the objective in \eqref{ll_obj1} is the same as in \eqref{eq:3}.



%\subsection{Notes on other works in transfer learning}
%
%***********THIS SECTION IS NOT A PART OF THE PAPER*****************
%
%When faced with a problem with a few labelled samples, one has three options: 
%\begin{enumerate}
%\item make better use of domain knowledge
%\item use unlabelled samples, this is semisupervised learning
%\item use labelled samples on a different problem
%\end{enumerate}
%
%The deep learning community has generally focused on the second option. Methods like Deep Boltzmann Machines (DBMs), Stacked Denoising Autoencoders (SDAs) or Sparse Coding (SC) can be used to learn generative representations from unlabelled samples. Then, these representations can be finetuned by standard backpropagation on the target problem.
%
%In a different strand of research, namely, multitask learning, one common approach has been learning representations such that they are useful for multiple tasks. In multitask learning, the tasks are fixed and the learner seeks to learn a model that generalizes well on unseen samples from these tasks. A more difficult case, is designing learners that learn to generalize to \textit{unseen tasks}. This is what is referred to as inductive bias learning, lifelong learning, learning to learn and other amusing names.
%
%Typically, multitask learners make what we referred to earlier as the task correspondence assumption. That is, during training or testing, the learner knows the identity of the task on which it is performing the training. 
%
%In 2000, Baxter provided sample complexity bounds for inductive bias learning. He also provided an algorithm. However, the algorithm Baxter provided is a multitask learning algorithm, this algorithm is the standard algorithm for multitask learning with neural networks.
%
%Since 2000, no work has shown how to create an inductive bias learner for neural networks. Our work fills this gap by presenting an algorithm. This algorithm learns representations such that they would minimize errors on unseen tasks. In other words, our algorithm optimizes the true objective Baxter's PAC bounds are related to. By learning representations to minimize errors on unseen tasks, our method falls into the third category. 
%
%\begin{table}
%    \begin{tabular}{llp{4cm}p{4cm}}
%    Method                                            & Inductive Bias & Hypothesis space                            & Complexity                                                            \\
%    ELLA                                              & Yes                    & Uses sparse coding as a regularizer         &  Computation time: $O(d^3 k^2) d$: data dimension $k$: sparse code size \\
%    OMTL                                              & No                     & Linear                                      &  space and time: $O(T^2) T$: number of tasks                           \\
%    Baxter                                            & No                     & Nonlinear                                   &  Linear in space in the number of tasks                               \\
%    Multitask Feature Learning                        & No                     & Linear, embeddable in Hilbert spaces        & Regularized Matrix Factorization                                      \\
%    Sparse coding for multitask\\
%     and transfer learning & Yes                    & Sparse coding, extendable to Hilbert spaces & sparse coding complexity, very similar to ELLA                        \\
%    GOMTL                                             & No                     & Sparse coding,                              & ~                                                                     \\
%    \end{tabular}
%\end{table}
%
%

